Cousins Of The Vendi Score: A Family Of Similarity-Based Diversity Metrics For Science And Machine Learning

Measuring diversity accurately is important for many scientific fields, including machine learning (ML), ecology, and chemistry. The Vendi Score was introduced as a generic similarity-based diversity metric that extends the Hill number of order q=1 by leveraging ideas from quantum statistical mechanics. Contrary to many diversity metrics in ecology, the Vendi Score accounts for similarity and does not require knowledge of the prevalence of the categories in the collection to be evaluated for diversity. However, the Vendi Score treats each item in a given collection with a level of sensitivity proportional to the item's prevalence. This is undesirable in settings where there is a significant imbalance in item prevalence. In this paper, we extend the other Hill numbers using similarity to provide flexibility in allocating sensitivity to rare or common items. This leads to a family of diversity metrics -- Vendi scores with different levels of sensitivity -- that can be used in a variety of applications. We study the properties of the scores in a synthetic controlled setting where the ground truth diversity is known. We then test their utility in improving molecular simulations via Vendi Sampling. Finally, we use the Vendi scores to better understand the behavior of image generative models in terms of memorization, duplication, diversity, and sample quality.

==> figures/molecules.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=\textwidth]{../figures/molecule_kernels}
  \caption{The kernel matrices for $250$ molecules sampled 
    from the \acrshort{HMM}, \acrshort{AAE}, and the original dataset, sorted
    lexicographically by \acrshort{SMILES} string representation.
    The samples have similar IntDiv scores,
    but the \acrshort{HMM} samples score much lower on \acrshort{VS}.
    The figure shows that the \acrshort{HMM} generates a number of exact duplicates. 
    \acrshort{VS} is able to capture the \acrshort{HMM}'s lack of diversity while IntDiv cannot.}
\label{fig:molecule_kernels}
\end{figure}
%\begin{figure}
%     \centering
%      \begin{minipage}[b]{0.34\textwidth}
%          \centering
%          \begin{tabular}{lcr}
%            \toprule
%            Model & IntDiv & $D_1^K$\\
%            \midrule
%            Original & 0.855 & 403.9\\
%            \midrule
%            AAE & 0.859 & 501.1\\
%            Char-RNN & 0.856 & 482.4\\
%            Combinatorial & 0.873 & 536.9\\
%            HMM & 0.871 & 250.9\\
%            JTN & 0.856 & 489.5\\
%            Latent GAN & 0.857 & 486.4\\
%            N-gram & 0.874 & 479.8\\
%            VAE & 0.856 & 475.3\\
%            \bottomrule
%          \end{tabular}
%          \captionof{table}{Internal Diversity score~\citep[IntDiv;
%            ][]{benhenda2017chemgan} and $D_1^K$ for generative models of
%            molecules. The HMM has one of the highest IntDiv scores, but a much
%            lower $D_1^K$ score compared to the other models.}
%          \label{tab:molecule_metrics}
%      \end{minipage}
%      \hfill
%      \begin{minipage}[b]{0.54\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{figures/molecule_kernels}
%          \caption{The kernel matrices for 250 molecules 
%            from the HMM, AAE, and the original dataset, sorted
%            lexicographically. The samples have similar IntDiv scores,
%            but the HMM samples score much lower on ${\ourmetric}$.
%            Visually, the HMM generates a number of groups of exact duplicates.}
%          \label{fig:molecule_kernels}
%      \end{minipage}
% \end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:

